Automata-Theoretic Characterisations of Branching-Time Temporal Logics

Characterisations theorems serve as important tools in model theory and can be used to assess and compare the expressive power of temporal languages used for the specification and verification of properties in formal methods. While complete connections have been established for the linear-time case between temporal logics, predicate logics, algebraic models, and automata, the situation in the branching-time case remains considerably more fragmented. In this work, we provide an automata-theoretic characterisation of some important branching-time temporal logics, namely CTL* and ECTL* interpreted on arbitrary-branching trees, by identifying two variants of Hesitant Tree Automata that are proved equivalent to those logics. The characterisations also apply to Monadic Path Logic and the bisimulation-invariant fragment of Monadic Chain Logic, again interpreted over trees. These results widen the characterisation landscape of the branching-time case and solve a forty-year-old open question.

==> Acknowledgments.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% Acknowledgments.tex                                                        %%
%%                                                                            %%
%% Copyright (C) 20xx, Fabio Mogavero.                                        %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file Acknowledgments.tex

\begin{section}*{Acknowledgments}

...

\end{section}

% End of file Acknowledgments.tex


==> Discussion.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% Discussion.tex                                                             %%
%%                                                                            %%
%% Copyright (C) 2024, Massimo Benerecetti, Laura Bozzelli, Fabio Mogavero,   %%
%%                     and Adriano Peron.                                     %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file Discussion.tex

\section{Discussion}

...

% End of file Discussion.tex


==> Figures.tex <==

%%****************************************************************************%%
%%                                                                            %%
%% Article Title                                                              %%
%%                                                                            %%
%% Figures.tex                                                                %%
%%                                                                            %%
%% Copyright (C) 20xx, Fabio Mogavero.                                        %%
%% All rights reserved.                                                       %%
%%                                                                            %%
%%****************************************************************************%%

% Begin of file Figures.tex

\AfterEndPreamble{

%%****************************************************************************%%

\newcommand{\fig}{
\begin{tikzpicture}[node distance = 5em, bend angle = 45]

  \node [cnode]
        (I)
        []
        {};
  \node []
        (X)
        [below of = I]
        {};

  \path[->]
    (I)   edge  [loop above]
                node [] {}
                ()
          edge  []
                node [] {}
                (X)
    ;

\end{tikzpicture}
}

%%****************************************************************************%%

}

% End of file Figures.tex

